An IoT Blockchain Architecture Using Oracles and Smart Contracts: the Use-Case of a Food Supply Chain

The blockchain is a distributed technology which allows establishing trust among unreliable users who interact and perform transactions with each other. While blockchain technology has been mainly used for crypto-currency, it has emerged as an enabling technology for establishing trust in the realm of the Internet of Things (IoT). Nevertheless, a naive usage of the blockchain for IoT leads to high delays and extensive computational power. In this paper, we propose a blockchain architecture dedicated to being used in a supply chain which comprises different distributed IoT entities. We propose a lightweight consensus for this architecture, called LC4IoT. The consensus is evaluated through extensive simulations. The results show that the proposed consensus uses low computational power, storage capability and latency.

==> 2_related.tex <==
In this section, first we discuss the related work regarding device scheduling and data quality in FEEL. Next, we illustrate the existing research gaps and motivate the need for designing a data-quality based scheduling algorithm for FEEL.

Among the first works to explore device selection is work in \cite{fedcs}, where authors mitigated the straggler problem by giving priority to end devices with good communication and computation capabilities. However, this method is not suitable in FEEL context, where datasets' distributions vary, as it discards UEs with larger and potentially more informative datasets. Several works proposed scheduling algorithms that aim to maximize the number of participating devices while optimizing used resources \cite{rh8,rh9}. For instance, authors in \cite{zeng_energy-efficient_2019} proposed an energy-efficient scheduling algorithm aiming to collect the maximum number of updates possible as a guarantee for the training speed. Another example is in \cite{yang_age-based_2020}, where authors study different scheduling strategies based on the wireless channel's state. Other works focus on the staleness of updates to calculate the priority \cite{yang_age-based_2020,xia_federated-learning-based_2021}, where higher priority is given to UEs that did not participate in previous rounds or have stale updates. Despite the variety of the scheduling algorithms in the literature, the design and evaluation of FEEL scheduling  under heterogeneous and uncertain dataset distributions remains a topic that is not well addressed, as data-quality issues are overlooked and under-explored.

To overcome the reliability problem,  several FL works use reputation systems for UEs selection, as UEs with high reputation are more likely to provide high quality data for the learning procedure. For instance, the authors in \cite{rh1} proposed a decentralized peer-to-peer approach to overcome the problem of unreliable UEs, where poisoning is prevented by verifying peer contributions to the model. However, due to stastical heterogeneity and high communication costs, P2P verification may not always be suitable. In \cite{rh3} and \cite{rh2}, the authors presented a blockchain-based reputation system for FL, where a  UE's reputation is traceable. In \cite{rh2}, the authors presented a reputation-based UE selection using subjective logic. This solution evaluates the reputation of UEs based on their past interactions with other task publishers in the network. Nonetheless, such approach relies on the willingness of several other similar task publishers to share their opinions.  
Based on our analysis of these works, we found that most of them did not consider the data heterogeneity when evaluating device reputation, and might not be suitable for realistic FEEL scenarios.
Consequently, we found it necessary to build a scheduling algorithm for FEEL that considers UEs datasets’ different properties ($i.e.,$ limited bandwidth, unbalanced/ non-IID data) alongside UEs reliability.















